One-Step weighting to generalize and transport treatment effect estimates to a target population

The problem of generalization and transportation of treatment effect estimates from a study sample to a target population is central to empirical research and statistical methodology. In both randomized experiments and observational studies, weighting methods are often used with this objective. Traditional methods construct the weights by separately modeling the treatment assignment and study selection probabilities and then multiplying functions (e.g., inverses) of their estimates. In this work, we provide a justification and an implementation for weighting in a single step. We show a formal connection between this one-step method and inverse probability and inverse odds weighting. We demonstrate that the resulting estimator for the target average treatment effect is consistent, asymptotically Normal, multiply robust, and semiparametrically efficient. We evaluate the performance of the one-step estimator in a simulation study. We illustrate its use in a case study on the effects of physician racial diversity on preventive healthcare utilization among Black men in California. We provide R code implementing the methodology.

==> onestep_sec1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec_introduction}

From the medical and social sciences to business and government research, the value of causal inferences from randomized experiments and observational studies depends on how well they generalize or transport to a target population of interest.
If treatment effects are modified by covariates whose distributions differ between the study sample and the target population, then effect estimates based on the study may not apply to the target \citep{degtiar2023review}.
Weighting methods show promise for generalizing and transporting treatment effect estimates from a study sample to a target population. 
Traditionally, these methods construct the weights by separately modeling and estimating unit-specific treatment assignment and study selection probabilities and then multiplying functions (e.g., inverses) of the estimated probabilities (e.g., \citealt{stuart2011use}, \citealt{tipton2018review}, \citealt{dahabreh2019generalizing}).  
If these models are correctly specified, then the weighted treatment and control groups will be balanced in expectation relative to the target population and the resulting weighted estimators will be unbiased for the target average treatment effect.

In practice, however, due to model misspecification, small samples, or sparse covariates, imbalances and biases can still exist. 
Additionally, as discussed by \cite{josey2021transporting} and \cite{lu2021you}, when the estimated treatment assignment or study selection probabilities are small, inverting or otherwise transforming them to obtain weights can magnify small prediction errors. 
The multiplicative structure of the two-step weights can further exacerbate this issue, resulting in highly variable and at times extreme weights where a few observations dominate the analysis.
In turn, this can produce unstable treatment effect estimators \citep{kang2007demystifying}.
%Furthermore, these methods require access to individual-level covariate data from the target population and do not directly apply to settings where only summary-level data are available, e.g., due to privacy concerns.

% There are recent works \textcolor{red}{that} address aspects of these issues. For randomized experiments, some methods use exact balancing (\citealt{dong2020integrative}) or approximate balancing (\citealt{lu2021you}) to construct the second-step weights (see also \citealt{hartman2015sample}). However, these methods do not readily apply to observational studies, where the first\textcolor{red}{-}step weights corresponding to the treatment assignment probabilities are unknown. Estimating these probabilities to construct the first step weights may lead to the same balance and stability issues mentioned before. For observational studies, \cite{josey2020calibration} proposes a full-calibration based approach that uses entropy balancing (\citealt{hainmueller2012balancing}, see also \citealt{zhao2017entropy}) in each step to obtain the corresponding weights. A related approach for randomized experiments is presented by \cite{josey2021transporting}. (***) However, these procedures \textcolor{red}{pursue} covariate balance exactly rather than approximately\textcolor{red}{,} and the resulting weights have a multiplicative structure, both of which can \textcolor{red}{diminish} the stability of the estimator. 

These concerns motivate the use of one-step weights for generalization and transportation; however, to our knowledge, the causal inference literature has yet to formalize and illustrate doing so.
In this paper, we fill this methodological and practical gap, and we justify, analyze, evaluate, and demonstrate a one-step weighting method for the generalization and transportation of effect estimates in both randomized experiments and observational studies, providing new insights into weighting methodology and its applications.
Building on existing covariate balancing approaches for causal inference, 
this method directly weights the treatment and control groups towards the target population in a single step, bypassing the need to estimate treatment and study selection probabilities separately and thereby avoiding a multiplicative structure of the weights.
\textcolor{red}{Our method connects to the recent calibration approaches by \cite{josey2021transporting}, \cite{li2021note} and \cite{lee2021improving}, while allowing for more flexible forms of covariate balance and accommodating more varied target populations.}
By balancing general transformations of the covariates, \textcolor{red}{the one-step method} does not require individual-level data from the target population, which may be unavailable for confidentiality reasons. \textcolor{red}{Instead}, summary statistics from the target are sufficient to execute the proposed method, which can be crucial in practice in settings where data access is limited.

Our paper proceeds as follows.
Section \ref{sec_setup} defines the notation and presents a framework for the generalization and transportation of causal inferences where the study and target populations are characterized in terms of generic probability distributions.
This framework is general and can encompass a number of generalization and transportation settings, including those  where the study population is nested within the target, those where study and target populations are disjoint, and those where the study and target populations partially overlap.
\textcolor{red}{As an example of the first case, consider the generalization of estimates from a randomized trial nested within a cohort study to the entire cohort; and as an example of the second, consider data from a randomized trial conducted in one state used to estimate the effects of treatment in another state.}
Motivated by this framework, 
Section \ref{sec_methods} proposes a method for estimating, in a single step, weights for transportation and generalization by targeting covariate balance while also avoiding highly-variable weights.
Section \ref{sec_asymptotic} derives the formal properties of this method, showing that, under regularity conditions, it yields a weighted estimator of the target average treatment effect that is consistent, asymptotically Normal, multiply robust, and semiparametrically efficient.
Section \ref{sec_simulation} assesses the empirical performance of the method in a simulation study and reveals how multiplicative weights, which are ubiquitous in practice, can underperform in finite samples.
An empirical case study in Section \ref{sec_empirical} illustrates the method with real data.
Section \ref{sec_remarks} concludes with some ideas for future directions.


==> onestep_sec3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Methods}
\label{sec_methods}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Weighting in one step}
\label{sec_onego}

In practice, in both inverse probability and inverse odds weighting, one often fits separate models for $e(\bm{x})$ and $\pi(\bm{x})$ and then multiplies the inverses (or functions) of the estimated probabilities to obtain the final weights. 
As discussed in Section \ref{sec_introduction}, such weights can be highly variable and fail to balance the covariates relative to the target population, producing biased and unstable estimators.
To address these issues, we formalize and use a weighting method that balances each treatment group toward the target in one step. 

For $z \in (0,1)$, let $m_z(\bm{x}) := E_{\mathbb{P}}\{Y(z)|\bm{X}=\bm{x}\}$ be the conditional mean function of $Y(z)$ given $\bm{X} = \bm{x}$. By Assumption \ref{assump1}(d), $m_z(\bm{x}) = E_{\mathbb{T}}\{Y(z)|\bm{X}=\bm{x}\}$, so $E_{\mathbb{T}}\{Y(z)\} = E_{\mathbb{T}}\{m_z(\bm{X})\}$. By Assumption \ref{assump1}(b), for normalized weights $w_i$, the bias of the H\'{a}jek estimator for $E_{\mathbb{T}}\{Y(z)\}$ is,
\begin{align} 
E_{\mathbb{P}}\left(\sum_{i:Z_i=z}w_i Y^{\mathrm{obs}}_i\right) - E_{\mathbb{T}}\left\{Y(z)\right\}  &=  E_{\mathbb{P}}\left[ \sum_{i:Z_i=z}w_i m_z(\bm{X}_i) - E_{\mathbb{T}}\{m_z(\bm{X})\}  \right].\label{eq:bias1}
\end{align}
In other words, weights that exactly balance the mean of $m_z(\bm{x})$ in treatment group $Z = z$ relative to $E_{\mathbb{T}}\{m_z(\bm{X})\}$ \textcolor{red}{(i.e., the mean of $m_z(\bm{x})$ in treatment group $Z = z$ after weighting becomes equal to $E_{\mathbb{T}}\{m_z(\bm{X})\}$)} completely remove the bias of $\sum_{i:Z_i=z}w_i Y^{\mathrm{obs}}_i$ as an estimator of $E_{\mathbb{T}}\{Y(z)\}$.
Assuming that $\Var_{\mathbb{P}}\left\{Y(z)|\bm{X} = \bm{x}\right\} = \sigma^2_z$ for $z \in (0,1)$, for all $\bm{x} \in \mathcal{X}$, we can compute the conditional variance of the weighted estimator as
\begin{equation}\label{eq:var1}
    \Var_{\mathbb{P}}\left(\sum_{i:Z_i=z}w_i Y^{\mathrm{obs}}_i \Big| \bm{X},\bm{Z} \right) = \sigma^2_z  \sum_{i:Z_i=z}w^2_i.
\end{equation}
This says that in order to obtain a stable H\'{a}jek estimator, it is crucial to have a set of weights with small $L_2$ norm.  
Together, Equations \ref{eq:bias1} and \ref{eq:var1} suggest the use of weights of small $L_2$ norm that balance the conditional mean functions $m_1(\bm{x})$ and $m_0(\bm{x})$ towards the target population of interest, and this guides our method.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Balancing towards the target population}
\label{sec_balancing}

Building on the minimal weights of \cite{wang2020minimal}, we solve the following convex optimization problem,
\begin{align}\label{minimal}
\argmin_{\bm{w}} \left\{  \sum_{i: Z_i=z}\psi(w_i) : \left|\sum_{i: Z_i=z} w_i B_k(\bm{X}_i) - \bar{B}^*_k    \right| \leq \delta_k, \; k = 1, 2, ..., K; \sum_{i:Z_i=z}w_i = 1
\right\},
\end{align}
where $B_k(\bm{X})$, $k = 1, 2, ..., K$ is a set of basis functions that spans $m_z(\bm{x})$, as motivated by Equation \ref{eq:bias1}, and $\psi$ is a smooth measure of the dispersion of the weights, such as their $L_2$ norm, as motivated by Equation \ref{eq:var1}.

The solution to \eqref{minimal} is the vector of weights $\bm{w}$ of minimum dispersion that approximately balances the weighted mean of the basis functions $B_k(\bm{X})$ in treatment group $Z = z$ relative to its mean in the target population, $\bar{B}_k^*$ \textcolor{red}{(i.e., the mean of $B_k(\bm{X})$ in treatment group $Z = z$ becomes approximately equal to $\bar{B}_k^*$ after weighting)}.
%The full vector $ \{\bar{B}_k^*$: $k = 1, ..., K \}$ is the covariate profile, and access to this summary measure from the target population is sufficient to execute the method.
\textcolor{red}{The full vector $ (\bar{B}_1^*,...,\bar{B}_K^*)^\top$ is the covariate profile, and access to this summary measure from the target population is sufficient to execute the method.}
The basis functions are flexible, ranging from main terms (which is sufficient for removing bias if $m_z(\bm{x})$ is linear in the covariates) to higher-order interactions (sufficient if $m_z(\bm{x})$ is linear in these interactions) to the basis functions corresponding to a particular kernel (sufficient if $m_z(\bm{x})$ lies in a reproducing kernel Hilbert space, RKHS).
See \cite{ben2021balancing} for a more detailed discussion.
Additional constraints in \eqref{minimal} can also force the weights to be non-negative and produce a sample-bounded estimator.
Finally, the parameters $\delta_k$, $k = 1, ..., K$, are set by the investigator, ultimately trading off bias for variance (see \citealt{chattopadhyay2020balancing} for a discussion and guidance). \textcolor{red}{In fact, leveraging connections between linear regression and weighting (\citealt{chattopadhyay2023implied}, \citealt{bruns2023augmented}),   
we show that with $\delta_k = 0$, $L_2$ objective, and without the non-negativity constraints, the one-step weighting estimator is equivalent to the linear regression imputation estimators in generalization and transportation problems (\citealt{dahabreh2019generalizing}, \citealt{dahabreh2020extending}). See Appendix \ref{sec_linearreg} in the Supplementary Materials for a proof.
}

In this way, the treatment groups are directly balanced relative to the target population in one step with weights of minimal dispersion that produce a stable estimator. This method is applicable to various generalization and transportation problems, including those where the study and target populations overlap and those where they are disjoint.

\textcolor{red}{We note that when the estimand is a weighted average treatment effect (WATE; see Table \ref{tab:estimands}), with standard choices of $h(\cdot)$ (e.g., $h(\bm{x}) = 1$ or $h(\bm{x}) = e(\bm{x})\{1-e(\bm{x})\}$), the two-step method boils down to a one-step weighting method that requires estimation of the propensity score only. With a correctly specified model for the propensity score, this method is expected to perform similarly to the proposed one-step method. Under model misspecification, the proposed one-step method may improve estimation efficiency since it explicitly controls the variability of the weights, while directly targeting covariate balance. 
}


==> onestep_sec4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Asymptotic properties}
\label{sec_asymptotic}

Implicitly, the one-step weighting method simultaneously models both the true inverse probability (or inverse odds) weights as well as the potential outcomes, the former via the dual optimization problem of \eqref{minimal} and the latter via the balancing conditions in \eqref{minimal}. 
In fact, since the one-step weights are obtained by solving \eqref{minimal} for the treated and control units separately, this method posits two separate models for the inverse probability weights of the treated and control units, and two separate models for the potential outcomes under treatment and control. These models are nonparametric in the sense that they uniformly approximate the true (weight or outcome) functions using a set of basis functions that grows with the sample size. 

{\color{red}
Assumptions \ref{assump2} and \ref{assump3} provide the exact specifications of these four models for generalization problems where the study sample is nested within a random sample of size $n^*$ from the target population. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}
\label{assump2}
\normalfont
The true inverse probability weights for group $Z=z$ satisfy $w^{\text{IP}}(\bm{x}) = n^* \rho'\{g^{*}_z(\bm{x})\}$ for all $\bm{x} \in \mathcal{\bm{X}}$, where  $g^*_z(\cdot)$ is a smooth function such that $\sup_{\bm{x} \in \bm{X}}|g^*_z(\bm{x}) - \bm{B}(\bm{x})^\top \bm{\lambda}^*_{1z}| = O(K^{-r_z})$ for some $\bm{\lambda}^*_{1z} \in \mathbb{R}^K$ and $r_z>1$.
\end{assumption}

\begin{assumption}\normalfont
The conditional mean function of the potential outcome under treatment $Z=z$ satisfies $\sup_{\bm{x}\in \mathcal{X}}|m_z(\bm{x}) - \bm{B}(\bm{x})^\top \bm{\lambda}^*_{2z}| = O(K^{-s_z}) $ for some $\bm{\lambda}^*_{2z} \in \mathbb{R}^K$ and $s_z>3/4$, with $||\bm{\lambda}^*_{2z}||_2 ||\bm{\delta}||_2 = o(1)$.
\label{assump3}
\end{assumption}

Assumption \ref{assump2} posits a functional form for the true inverse propensity weights through the function $\rho(\cdot)$ obtained from the dual problem of \eqref{minimal} (see \eqref{dual1} in the Supplementary Materials) and a smooth function $g^*_z(\cdot)$. It states that $g^*_z(\cdot)$ can be uniformly well-approximated by the vector of basis functions $\bm{B}(\cdot)$. Akin to nonparametric sieve estimation (\citealt{andrews1991asymptotic}, \citealt{newey1997convergence}; see also \citealt{fan2016improving}), here the number of basis functions $K$ grows with $n^*$. 
$g^*_z(\cdot)$ can incorporate a large number of flexible basis functions, including interactions and higher order transformations of the covariates. 
In particular, Assumption \ref{assump2} is satisfied in the parametric case when $g^*_z(\cdot)$ is a linear combination of a finite number of basis functions in $\bm{B}(\cdot)$. 

Similarly, Assumption \ref{assump3} states that the conditional mean function $m_z(\cdot)$ can be uniformly approximated by the basis functions $\bm{B}(\cdot)$ (i.e., the one-step balancing weights balance the appropriate covariate functions). In particular, it is satisfied when $m_z(\cdot)$ is a linear combination of the functions in $\bm{B}(\cdot)$. The condition $||\bm{\lambda}^*_{2z}||_2 ||\bm{\delta}||_2 = o(1)$ is a technical requirement that ensures that the coefficients of $\bm{B}(\cdot)$ do not dominate the overall degree of approximate balance as the number of basis functions goes to infinity.

Leveraging these four assumptions and some additional regularity conditions, we can establish multiple robustness of the one-step H\'{a}jek estimator of the target average treatment effect. At a high level, these regularity conditions pertain to the dual objective function and basis functions that are used to approximate the true inverse probability weights and the potential outcomes. We state them formally in Assumption \ref{assump4} below.

\begin{assumption} \normalfont
\label{assump4}
For $z \in \{0,1\}$, 
\begin{enumerate}[label=(\alph*)]

%\item There exist constants $c_1$ and $c_2$ with $c_1<c_2<0$ such that $c_1 \leq n^*\rho{''}(v) \leq c_2$ for all $v$ in a neighborhood of $\bm{B}(\bm{x})^\top \bm{\lambda}^*_{1z}$.

\item There exist constants $c_0$, $c_1$, $c_2$ with $0<c_0<1/2$ and $c_1<c_2<0$, such that $c_1 \leq n^*\rho{''}(v) \leq c_2$ for all $v$ in a neighborhood of $\bm{B}(\bm{x})^\top \bm{\lambda}^*_{1z}$. Also, $c_0 \leq 1/(n^*\rho'(v)) \leq 1-c_0$ for all $v = \bm{B}(\bm{x})^\top \bm{\lambda}$, $\bm{x} \in \mathcal{X}$, $\bm{\lambda}$. % range of x check
    
    \item $\sup\limits_{x \in \mathcal{X}}||\bm{B}(\bm{x})||_2 \leq CK^{1/2}$ and $||E_{\mathbb{T}}\{\bm{B}(\bm{X}) \bm{B}(\bm{X})^\top\}||_F \leq C$, for some constant $C>0$, where $||\cdot||_F$ denotes the Frobenius norm.
  
    \item $K = O\{(n^*)^\alpha\}$ for some $0<\alpha<2/3$.
    
    \item For some constant $C>0$, $\lambda_{\text{min}}\Big[ E_{\mathbb{T}}\{D\mathbbm{1}(Z = z)\bm{B}(\bm{X})\bm{B}(\bm{X})^\top\}\Big]>C$, where $\lambda_{\min}(\bm{A})$ denotes the smallest eigenvalue of $\bm{A}$.
    
    \item $||\bm{\delta}||_2 = O_P\left[K^{1/4}\left\{(\log K) / n^*\right\}^{1/2} + K^{- r_z + 1/2}\right]$.
\end{enumerate}
\end{assumption}

The conditions in Assumption \ref{assump4} are similar to the technical conditions in Assumption 1 of \cite{wang2020minimal} and Assumption 4.1 in \cite{fan2016improving}. In particular, Assumption \ref{assump4}(a) bounds the slope and curvature of the function $\rho(\cdot)$, allowing us to translate the convergence of the dual solution to the convergence of the weights. This condition is satisfied for typical choices of convex objective functions $\psi(\cdot)$, e.g., those corresponding to entropy balancing \citep{hainmueller2012balancing} and stable balancing weights \citep{zubizarreta2015stable}.
Assumption \ref{assump4}(b) restricts the rate of growth of the norm of the basis functions, and \ref{assump4}(c) specifies the rate of growth of the number of basis functions $K$ relative to $n^*$. Assumption \ref{assump4}(d) is a technical condition required to ensure non-singularity of the covariance matrices of the basis functions within each treatment group. Finally, \ref{assump4}(e) controls the degree of approximate balancing in terms of $K$ and $n^*$.

Given the above assumptions, Theorem \ref{thm_consistency} establishes multiple consistency conditions for the one-step H\'{a}jek estimator of the TATE.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}[Consistency] \normalfont
\label{thm_consistency}
Suppose that Assumptions \ref{assump1} and \ref{assump4} hold. Then
the one-step H\'{a}jek estimator $\hat{\tau} = \sum_{i:Z_i=1}\widehat{w}_iY^{\text{obs}}_i - \sum_{i:Z_i=0}\widehat{w}_iY^{\text{obs}}_i$ is consistent for the target average treatment effect $\tau$ if any of the following conditions are satisfied.
\begin{enumerate}[label =(\alph*)]
%\itemsep-.5em
%\item[]
 \item The models for the inverse probability weights of the treated and control units are both correctly specified.
 \item The models for the potential outcomes under treatment and control are both correctly specified.
 \item The models for the inverse probability weights of the treated units and the potential outcomes under control are both correctly specified. 
 \item The models for the inverse probability  weights of the control units and the potential outcomes under treatment are both correctly specified. 
\end{enumerate}
\end{theorem}

Thus, in a similar way to multiply robust estimators,  $\hat{\tau}$ admits multiple conditions for consistency, where each condition requires a suitable approximation of the implied models for the inverse probability weights, the potential outcomes, or a combination of the two. 

Finally, if all the aforementioned four models are correctly specified, then under some additional regularity conditions, $\hat{\tau}$ is asymptotically Normal and semiparametrically efficient for the target average treatment effect $\tau$ (\citealt{robins1995semiparametric}). At a high level, these regularity conditions pertain to the complexity of the unknown inverse probability weight and potential outcome mean functions. We state them formally in Assumption \ref{assump5} below.

%\setcounter{assumption}{2}
\begin{assumption}\normalfont
\label{assump5}
For $z \in \{0,1\}$, 
\begin{enumerate}[label=(\alph*)]

\item $E_{\mathbb{T}}\{Y^2(z)\}<\infty$.

\item Let $g^*_z(\cdot) \in \mathcal{G}_z$. $\mathcal{G}_z$ satisfies $\log N_{[]}\{\epsilon, \mathcal{G}_z, L_2(P)\} \leq C_1(1/\epsilon)^{1/k_1}$ for some constants $C_1>0$ and $k_1>1/2$, where $N_{[]}\{\epsilon, \mathcal{G}_z, L_2(P)\}$ is the covering number of $\mathcal{G}_z$ by epsilon brackets.
    
\item Let $m_z(\cdot) \in \mathcal{M}_z$. $\mathcal{M}_z$ satisfies $\log N_{[]}\{\epsilon, \mathcal{M}_z, L_2(P)\} \leq C_2(1/\epsilon)^{1/k_2}$ for some constants $C_2>0$ and $k_2>1/2$, , where $N_{[]}\{\epsilon, \mathcal{M}_z, L_2(P)\}$ is the covering number of $\mathcal{M}_z$ by epsilon brackets.

\item $(n^{*})^{\{2(r_z + s_{z} - 0.5)\}^{-1}} = o(K)$, where $r_z, s_z$ are the constants in assumptions 2 and 3, respectively. 
    
\end{enumerate}
\end{assumption}

The conditions in Assumption \ref{assump5} are similar to Assumption \ref{assump2} in \cite{wang2020minimal} and Assumption 4.1 in \cite{fan2016improving}. In particular, Assumption \ref{assump5}(a) ensures existence of the second moment of $Y(z)$ with respect to the target distribution. Assumptions \ref{assump5}(b) and (c) control the complexity of the function classes $\mathcal{G}_z$ and $\mathcal{M}_z$. Finally, Assumption \ref{assump5}(d) puts further restriction on the growth rate of the number of basis functions $K$ as a function of $n^*$. 


Theorem \ref{thm_normality} establishes asymptotic Normality and semiparametric efficiency of the one-step H\'{a}jek estimator of the TATE.

}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}[Asymptotic normality and semiparametric efficiency]\normalfont
\label{thm_normality}
Suppose that the study sample is nested within a random sample of size $n^*$ from the target population and that Assumptions 2-5 hold. Then, as $n^*$ tends to infinity, $(n^*)^{1/2}(\widehat{\tau} - \tau)$ converges in distribution to a Normal random variable with mean 0 and variance $V^*_\tau = E_{\mathbb{T}}(\sigma^2_1(\bm{X})/ \{\pi(\bm{X})e(\bm{X})\} + {\sigma^2_0(\bm{X}) / [\pi(\bm{X})\{1-e(\bm{X})\}]} + \{m_1(\bm{X})-m_0(\bm{X}) - \tau\}^2 )$, where $\sigma^2_z(\bm{x}) = \Var_{\mathbb{T}}\{Y(z)|\bm{X}=\bm{x}\}$ for $z \in (0,1)$.
\end{theorem}
\textcolor{red}{For generalization problems in nested study settings, $V^*_\tau$ is shown to be precisely the semiparametric efficiency bound for the TATE, regardless of whether the study is randomized or observational (\citealt{li2021note}; see also \citealt{lee2021improving}). Theorem \ref{thm_normality} states that the one-step estimator achieves the semiparametric efficiency bound.}

{\color{red}
We conclude this section with a couple of remarks. First, the asymptotic properties are derived under the assumption that the potential outcomes are homoscedastic. However, as shown in \cite{hirshberg2021augmented}, even under heteroscedasticity, the desired asymptotic properties hold for a similar class of balancing estimators. The rationale is as follows. The inverse probability (IP) weights are the unique set of weights that balance all measurable functions of the covariates in expectation. Since the basis functions balanced by the one-step approach are allowed to grow flexibly with the sample size, in large samples, the one-step weights come close to exhibiting the same balancing properties as the IP weights.
The uniqueness property of the IP weights then implies that, even under heteroscedasticity, the one-step weights end up estimating the IP weights. This result in turn implies that the desired asymptotic properties hold for the one-step weights. We also investigate the finite sample performance of the one-step estimator under heteroscedasticity using a simulation study; see Appendix \ref{sec_simu_hetro} in the Supplementary Materials for details.

Second, the asymptotic properties are derived without explicitly constraining the weights to be non-negative. Nevertheless, with these non-negativity constraints, the one-step estimator is expected to exhibit similar asymptotic behavior as that without the constraints. This phenomenon stems from the observation that under the overlap conditions in Assumptions 1(a) and 1(c), the one-step weights with and without the non-negativity constraints are asymptotically equivalent. More formally, Assumptions 1(a) and 1(c) imply that the support of the covariates in group $Z = z$ is the same as that in the target population. 
    %Hence, with a large enough sample size, the target profile  $(\bar{B}^*_1,...,\bar{B}^*_K)^\top$ tends to lie within the convex hull of the data $\{(B_1(\bm{X}_i),...,B_K(\bm{X}_i))^\top:Z_i =z\}$, allowing us to sufficiently balance these functions relative to the target profile without extrapolation (i.e., without requiring negative weights). 
    In other words, in large samples, the solutions to (7) tend to be non-negative, coinciding with the solutions where (7) explicitly includes the non-negativity constraints. See Proposition 1 in \cite{zhao2016entropy} for a related discussion in the context of entropy balancing.

}

==> onestep_sec5.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Simulation study}
\label{sec_simulation}
We evaluate the performance of the one-step weights in a simulation study for generalizing treatment effect estimates from a study to a larger cohort in which the study is nested.
We consider both randomized and observational study settings.

Our design builds on \cite{kang2007demystifying}.
There are four independent unobserved covariates distributed as $U_1, U_2, U_3, U_4 \sim \mathcal{N}(0, 1)$, and four observed covariates generated as $X_1 = \exp(U_1/2)$, $X_2 = U_2/\{1 + \exp(U_1)\} + 10$, $X_3 = (U_1U_3/25 + 0.6)^3$, and $X_4 = (U_2 + U_4 + 20)^{2}$.
$D$ is the binary indicator for selection into the study, and $Z$ is the binary treatment indicator.
The true model for the probability of selection into the study is $\mathrm{pr}(D = 1 | \bm{U}) = \text{expit}(-U_1 + 0.5 U_2 - 0.25 U_3 - 0.1 U_4)$ so that, marginally, $\mathrm{pr}(D = 1)  = 0.5$. 
The total cohort size is 1000.
For the randomized study setting, $\mathrm{pr}(Z = 1|\bm{U}) = 0.5$, and for the observational setting, $\mathrm{pr}(Z=1|\bm{U}) = \text{expit}(U_1 + 2U_2 - 2U_3 - U_4)$. 

There is one control potential outcome model, $Y(0) = 210 + 27.4 U_1 + 13.7 U_2 + 13.7 U_3 + 13.7 U_4 + \epsilon_0$, where $\epsilon_0 \sim \mathcal{N}(0, 5^2)$, and there are three treatment potential outcome models: Model 1 is given by $Y(1) = 210 + 27.4 U_1 + 13.7 U_2 + 13.7 U_3 + 13.7 U_4 + \epsilon_1$; Model 2 by $Y(1) = 210 + 41.1 U_1 + 13.7 U_2 + 13.7 U_3 + 13.7 U_4 + \epsilon_1$; and Model 3 by $Y(1) = 210 + 41.1 U_1 + 27.4 U_2 + 27.4 U_3 + 13.7 U_4 + \epsilon_1$; where $\epsilon_1 \sim \mathcal{N}(0,5^2)$.
Thus, the target average treatment effect is $0$ in all cases, but the degree of treatment effect heterogeneity varies across the models\textcolor{red}{, which allows us to compare methods' performance under varying degrees of treatment effect heterogeneity and scenarios where the variables determining such heterogeneity are accounted for or not in the adjustments.}
For Model 1, there is no heterogeneity; for Model 2, there is heterogeneity by $U_1$; and for Model 3, there is heterogeneity by $U_1$, $U_2$, and $U_3$.
Specifically, for Model 1, $E\{Y(1) - Y(0) | \bm{U}\} = 0$, for Model 2, $E\{Y(1) - Y(0) | \bm{U}\} = 13.7 U_1$, and for Model 3, $E\{Y(1) - Y(0) | \bm{U}\} = 13.7 U_1 + 13.7 U_2 + 13.7 U_3$.

We compare three versions of one-step weighting to three versions of two-step weighting.
The first one-step method balances the mean of the first observed covariate only, the second balances the means of all of the observed covariates, and the third balances the means of all of the unobserved covariates.
For the one-step methods, \textcolor{red}{we find the weights that solve \eqref{minimal}}.
A variation of the tuning algorithm in \cite{chattopadhyay2020balancing} is used to select the imbalance tolerances, where imbalances are computed relative to the target covariate profile.
\textcolor{red}{Moreover, in \eqref{minimal}, we minimize the $L_2$ norm of the weights.
%, although related works on balancing weights have shown that the performances of these weighting methods are relatively insensitive to the choice of the objective function (see, e.g., \citealt{wang2020minimal}, \citealt{lee2021improving}). 
Our choice stems from Equation \ref{eq:var1}, which shows that the variance of the weighted estimator is directly linked to the $L_2$ norm of the weights.}

The two-step methods \textcolor{red}{fit separate models for the two unknown functions, the probability of sample selection and the probability of treatment assignment given covariates, and plug the estimated probabilities from these models into \eqref{eq:ipw_identify2} to compute the weights.}
These models are logistic regressions of the study selection indicator on covariates and additionally of the treatment indicator on covariates in the observational study setting, where the first two-step method only uses the first observed covariate in the regression, the second uses all of the observed covariates, and the third uses all of the unobserved covariates.
The third two-step and one-step methods are correctly-specified, while the others are misspecified.

Table \ref{tab:Tab2} shows the root-mean-squared errors of the H\'{a}jek estimators, based on 800 simulations.
The one-step weights outperform the two-step weights across the three outcome models in both the randomized and observational study settings. 
In the randomized study, the one-step weights reduce the root-mean-squared error relative to the corresponding two-step estimators by $86\%$, on average. 
In the observational study, the one-step estimators achieve $70\%$ smaller root-mean-squared error relative to the corresponding two-step estimators, on average. 
In particular, the root-mean-squared errors under the correctly specified one-step methods are an order of magnitude smaller than those under the correctly specified two-step methods. \textcolor{red}{A similar pattern is observed in settings that allow for heteroscedasticity of the potential outcome models; see Appendix \ref{sec_simu_hetro} in the Supplementary Materials for details.}

\begin{table}[H]
\singlespacing
\centering
\caption{\label{tab:Tab2} Root-mean-squared error of the H\'{a}jek estimator of the target average treatment effect using different weighting methods in both the randomized and observational study settings.}
\begin{tabular}{lrrrrrrr}
                  & \multicolumn{3}{c}{Randomized Study Setting} &  & \multicolumn{3}{c}{Observational Study Setting} \\ \cline{2-4} \cline{6-8} 
                  & Outcome       & Outcome       & Outcome      &  & Outcome        & Outcome        & Outcome       \\
Weighting Method  & Model 1       & Model 2       & Model 3      &  & Model 1        & Model 2        & Model 3       \\ \hline
Two-Step 1 & 17.47         & 21.80         & 23.53        &  & 22.55          & 24.76          & 24.96         \\
One-Step 1 & 2.91          & 3.17          & 4.40         &  & 9.18           & 8.64           & 7.58          \\
Two-Step 2 & 19.00         & 23.70         & 25.23        &  & 42.47          & 41.44          & 45.72         \\
One-Step 2 & 2.26          & 2.53          & 3.27         &  & 17.32          & 16.38          & 24.16         \\
Two-Step 3 & 4.75          & 5.58          & 6.09         &  & 9.11           & 10.59          & 12.43         \\
One-Step 3 & 0.54          & 0.70          & 0.91         &  & 0.73           & 0.90           & 1.14      \\
\hline
\end{tabular}
\end{table}

These improvements are at least partially driven by the high variability and extremity of the two-step weights. 
Figure \ref{fig:ess} shows how the effective sample sizes and maximum normalized weights vary across simulations.
The effective sample size relates to the variance of the weights, where, roughly, higher variance corresponds to lower effective sample size (see, e.g., \citealt{chattopadhyay2020balancing}). Similarly, the maximum normalized weight provides a measure of the extremity of the weights.

\begin{centering}
\begin{figure}[H]
\centering
\caption{Effective sample sizes and maximum normalized weights across weighting methods in both the randomized and observational study settings.}\label{fig:ess}
\includegraphics[scale=0.9]{graphics/WeightsPlot.pdf}
\end{figure}
\end{centering}

In the randomized study, the one-step method leads to a $43\%$ improvement in the effective sample size compared to the two-step method on average.
In the observational study, the one-step method leads to an $87\%$ improvement in the effective sample size over the two-step method on average: more than double its improvement in the randomized study. 
Here, we see how the multiplicative structure of the two-step weights exacerbates the problem of extreme weights when there is less overlap across treatment groups, as is the case in the observational setting as compared to the randomized one.
Finally, in both study settings, the maximum normalized weights under the two-step method tend to be more extreme than those under the one-step method, particularly for the observational study. 
In some cases, the most extreme normalized weight under the two-step method is very close to one, signifying that nearly all information used to construct the treatment effect estimator comes from a single unit.


In the current simulation setup, the study population is contained in the target population. 
\textcolor{red}{To investigate the performance of the one-step method for other target populations, we consider another simulation study where the study and target populations are disjoint (see Appendix \ref{appendix_simulation} in the Supplementary Materials).}
%In the Supplementary Materials, we consider another simulation study where the study and target populations are disjoint. 
Here too, the one-step methods are shown to outperform the two-step methods.
%\textcolor{red}{Finally, for a target population corresponding to a weighted average treatment effect (WATE; see Table \ref{tab:estimands}), with standard choices of $h(\cdot)$ (e.g., $h(\bm{x}) = 1$ or $h(\bm{x}) = e(\bm{x})\{1-e(\bm{x})\}$), the two-step method boils down to a one-step weighting method that requires estimation of the propensity score only. With a correctly specified model for the propensity score, this method is expected to perform similarly to the proposed one-step method. Under model misspecification, the proposed one-step method may improve estimation efficiency since it explicitly controls the variability of the weights, while directly targeting covariate balance. }


